Elemental Abundances of Cool Stars: A Spectroscopic Framework Applied to Five Planet-Host Stars

Stellar elemental abundances provide important constraints on the chemical environments from which planets form. M and late-K dwarfs are prime targets for the characterization of small exoplanets, yet their complex spectra make accurate elemental abundance measurements challenging. In this work, we present a spectral synthesis-based framework to derive detailed abundances for cool stars from high-resolution, near-infrared spectra. We apply our framework to SPIRou YJHK spectra of five planet-host stars--GJ 9827, K2-18, TOI-1201, TOI-1685, and Barnard's Star--and derive abundances of C, O, Na, Mg, Al, Si, K, Ca, Ti, Cr, Mn, and Fe for all five stars, plus Sc, V, and Ni for a subset, with typical uncertainties of $\lesssim 0.1$ dex. Our recovered metallicities and elemental abundances are broadly consistent with expected trends and previous literature analyses of these stars. We derive stellar ratios of C/O, Mg/Si, Fe/Mg, and Fe/O and find that all five systems are broadly consistent with solar ratios, with the exception of the metal-poor Barnard's Star ([M/H] $= -0.33 \pm 0.06$ dex), which is substantially iron-poor ([Fe/H] $= -0.722 \pm 0.085$ dex). Our results establish stellar chemical baselines for interior structure and atmospheric studies of these planetary systems with the Hubble Space Telescope (HST) and James Webb Space Telescope (JWST), while highlighting the remaining model-dependent limitations of precise abundance analyses for cool stars.

==> Tables/linelist_complete.tex <==
\begin{table}[htbp]
\centering
\caption{Complete linelist and line-by-line abundances}
\label{tab:complete_lines}
\begin{tabular}{ccccccc}
\hline
Wavelength [nm] & Species & GJ 9827 & K2-18 & TOI-1201 & TOI-1685 & Barnard's Star \\
\hline
1078.19722 & Al 1 &  &  & -0.02 &  &  \\
1087.29300 & Al 1 & -0.11 &  &  &  &  \\
1089.16740 & Al 1 & -0.15 &  &  &  &  \\
1125.31943 & Al 1 & -0.33 &  &  &  & -0.41 \\
1125.48831 & Al 1 & -0.26 &  & -0.03 &  & -0.52 \\
1312.34148 & Al 1 & -0.36 & 0.10 & -0.13 & 0.06 & -0.25 \\
1315.07514 & Al 1 & -0.39 & 0.05 & -0.03 & 0.14 & -0.29 \\
1671.89078 & Al 1 & -0.31 & 0.17 & -0.08 & -0.00 &  \\
1675.05117 & Al 1 & -0.39 & -0.19 &  &  & -0.15 \\
1676.33154 & Al 1 & -0.26 & 0.15 & 0.05 &  &  \\
2109.29737 & Al 1 & -0.19 &  &  &  &  \\
2116.37094 & Al 1 & -0.24 &  &  &  &  \\
2292.92232 & CO 1 & -0.19 &  & 0.22 & 0.16 & -0.40 \\
2293.01808 & CO 1 & -0.20 & 0.22 &  & 0.16 & -0.39 \\
2293.14330 & CO 1 & -0.18 &  &  &  & -0.50 \\
2293.31778 & CO 1 & -0.19 & 0.22 &  & 0.11 & -0.35 \\
2293.48421 & CO 1 &  & 0.30 &  &  &  \\
2293.53404 & CO 1 & -0.23 & 0.14 &  &  & -0.44 \\
2293.72435 & CO 1 & -0.20 & 0.09 & 0.07 & -0.05 &  \\
2293.78470 & CO 1 & -0.26 & 0.15 & -0.10 & 0.17 & -0.31 \\
2294.00382 & CO 1 & -0.25 & 0.31 & -0.02 & 0.06 & -0.27 \\
2294.07627 & CO 1 &  & 0.28 & 0.06 &  & -0.16 \\
2294.32729 & CO 1 & -0.18 &  & -0.11 &  & -0.34 \\
2294.40766 & CO 1 & -0.24 & 0.27 & -0.00 & 0.20 &  \\
2294.69197 & CO 1 & -0.30 & 0.07 & 0.02 &  & -0.30 \\
2294.77774 & CO 1 & -0.21 & 0.33 & -0.09 &  & -0.31 \\
2295.09983 & CO 1 &  & 0.25 & 0.02 & 0.13 & -0.29 \\
2295.18891 & CO 1 & -0.24 & 0.25 & -0.04 & 0.15 & -0.38 \\
2295.54708 & CO 1 & -0.20 & 0.19 &  & 0.09 & -0.42 \\
2295.64052 & CO 1 & -0.13 & 0.31 & 0.08 &  & -0.32 \\
2296.03694 & CO 1 & -0.13 & 0.41 & -0.06 &  &  \\
2296.13066 & CO 1 &  & 0.18 & -0.12 &  & -0.24 \\
2296.56968 & CO 1 &  & 0.14 & 0.01 &  & -0.20 \\
2296.66047 & CO 1 & -0.28 & 0.26 & 0.03 & 0.27 &  \\
2297.14530 & CO 1 &  &  &  & 0.27 &  \\
2297.22979 & CO 1 &  & 0.26 & 0.03 &  & -0.15 \\
2297.76452 & CO 1 &  & 0.23 &  &  &  \\
2297.84092 & CO 1 & -0.18 & 0.44 & 0.27 &  &  \\
2298.42036 & CO 1 & -0.12 & 0.32 & 0.10 &  &  \\
2298.49125 & CO 1 & -0.16 &  &  &  &  \\
2299.18052 & CO 1 & -0.16 & 0.34 & 0.02 & 0.29 & -0.37 \\
2299.91104 & CO 1 & -0.19 &  &  &  & -0.24 \\
2300.68267 & CO 1 & -0.21 & 0.35 & 0.03 & 0.28 & -0.19 \\
2301.49707 & CO 1 & -0.14 & 0.17 & 0.01 & 0.20 & -0.34 \\
2302.35191 & CO 1 & -0.20 & 0.42 & 0.06 & 0.39 &  \\
2303.24720 & CO 1 & -0.21 & 0.34 & 0.06 & 0.15 &  \\
2304.17384 & CO 1 & -0.16 & 0.41 & 0.25 &  &  \\
2305.14548 & CO 1 & -0.29 & 0.29 & 0.12 & 0.44 & 0.14 \\
2305.24287 & CO 1 & -0.16 &  &  &  &  \\
2306.15634 & CO 1 &  & 0.47 & 0.07 &  &  \\
2307.21130 & CO 1 & -0.25 & 0.50 & 0.22 &  &  \\
2307.38786 & CO 1 & -0.16 &  &  &  &  \\
2308.30149 & CO 1 & -0.21 & 0.11 & 0.06 & 0.36 &  \\
2309.43426 & CO 1 & -0.27 &  &  &  &  \\
2310.60760 & CO 1 & -0.21 &  & 0.25 &  &  \\
2311.82152 & CO 1 & 0.23 & 0.39 &  &  & -0.15 \\
2313.07471 & CO 1 & -0.21 & 0.41 & 0.09 & 0.27 &  \\
2314.36837 & CO 1 & -0.17 & 0.34 & 0.11 &  &  \\
2315.70289 & CO 1 & -0.18 & 0.44 & 0.25 &  &  \\
2317.08092 & CO 1 &  & 0.38 & 0.14 &  &  \\
2318.49670 & CO 1 & -0.25 & 0.40 & 0.10 &  &  \\
2319.95205 & CO 1 & -0.16 & 0.35 & 0.25 &  &  \\
2321.44820 & CO 1 & -0.19 & 0.34 & 0.06 &  &  \\
2322.04829 & CO 1 & -0.27 & 0.35 & -0.04 &  & -0.42 \\
2322.10340 & CO 1 &  & 0.23 & 0.15 &  &  \\
2322.21518 & CO 1 & -0.25 & 0.27 &  &  & -0.49 \\
2322.32467 & CO 1 & -0.22 & 0.18 & 0.03 &  &  \\
2322.38170 & CO 1 & -0.32 & -0.00 & -0.08 & 0.11 & -0.50 \\
2322.50850 & CO 1 & -0.28 & 0.38 & 0.14 & 0.35 &  \\
2322.57950 & CO 1 &  & 0.19 & -0.03 &  &  \\
2322.72936 & CO 1 &  & 0.22 & 0.08 & 0.13 & -0.02 \\
2322.81648 & CO 1 & -0.27 & 0.01 & -0.01 &  & -0.29 \\
2322.99063 & CO 1 & -0.30 & 0.29 & 0.05 & 0.23 & -0.30 \\
2323.09578 & CO 1 &  & 0.33 & 0.05 &  &  \\
2323.30404 & CO 1 & -0.09 & 0.20 & 0.23 & 0.19 &  \\
2323.41304 & CO 1 & -0.33 & 0.29 & 0.23 &  &  \\
2323.65388 & CO 1 & -0.22 & 0.04 & -0.00 & 0.15 & -0.39 \\
2323.77270 & CO 1 & -0.32 & 0.22 &  & 0.31 & -0.41 \\
2324.17551 & CO 1 & -0.26 &  & 0.13 &  &  \\
2324.48368 & CO 1 &  &  &  & 0.23 &  \\
2324.60343 & CO 1 &  &  & 0.20 & 0.38 &  \\
2324.95984 & CO 1 & -0.17 &  & 0.11 &  &  \\
2325.10364 & CO 1 & -0.27 & 0.13 & -0.00 & 0.15 & -0.20 \\
2325.48287 & CO 1 & -0.23 & 0.24 & 0.25 &  &  \\
2325.62984 & CO 1 &  & 0.24 &  & 0.20 &  \\
2326.04880 & CO 1 & -0.27 &  &  &  &  \\
2326.19152 & CO 1 & -0.22 & 0.30 & 0.04 &  & -0.39 \\
2326.65805 & CO 1 & -0.20 & 0.31 & 0.07 &  & -0.19 \\
2326.80260 & CO 1 & -0.20 & 0.40 & 0.23 &  &  \\
2327.30865 & CO 1 & -0.20 & 0.26 &  & 0.23 &  \\
2327.45256 & CO 1 &  & 0.40 & 0.10 & 0.27 &  \\
2327.84731 & CO 1 & -0.24 & 0.29 & 0.01 &  &  \\
2328.00475 & CO 1 & -0.14 &  & 0.25 &  &  \\
2328.14191 & CO 1 & -0.29 &  & 0.21 &  &  \\
2328.75016 & CO 1 &  &  & 0.01 &  &  \\
2328.87268 & CO 1 & -0.30 &  &  &  & -0.15 \\
2329.54597 & CO 1 & -0.14 & 0.33 & 0.07 &  & 0.00 \\
2329.64348 & CO 1 & -0.18 & 0.37 & 0.12 &  &  \\
2330.35800 & CO 1 & -0.09 &  & 0.25 & 0.23 &  \\
2330.45719 & CO 1 & -0.26 & 0.37 & 0.06 & 0.26 &  \\
2331.30455 & CO 1 & -0.18 & 0.35 & 0.06 & 0.29 & -0.08 \\
2332.20389 & CO 1 & -0.24 &  & 0.00 &  &  \\
2333.13443 & CO 1 & -0.18 &  & 0.00 &  & -0.37 \\
2334.12224 & CO 1 &  & 0.42 & 0.24 &  &  \\
2335.14134 & CO 1 &  & 0.38 & 0.24 & 0.23 &  \\
2336.20026 & CO 1 &  & 0.22 & 0.03 &  & -0.14 \\
2336.77452 & CO 1 & -0.19 &  & -0.01 &  &  \\
2337.30000 & CO 1 & -0.24 & 0.22 & -0.09 &  & -0.15 \\
2338.44247 & CO 1 &  & 0.35 &  &  &  \\
2338.68255 & CO 1 & -0.12 &  &  &  &  \\
2340.63436 & CO 1 & 0.64 &  &  &  &  \\
2340.85022 & CO 1 & -0.27 &  & 0.25 &  &  \\
2341.10301 & CO 1 & -0.24 &  &  &  &  \\
2342.11765 & CO 1 &  & 0.29 & 0.05 & 0.26 & -0.05 \\
2342.42885 & CO 1 & -0.13 &  &  &  &  \\
2342.62910 & CO 1 & -0.10 &  &  &  & -0.25 \\
2343.42541 & CO 1 & -0.26 &  & 0.14 &  &  \\
2344.77756 & CO 1 &  &  & 0.25 &  &  \\
2346.16450 & CO 1 & -0.11 & 0.48 & 0.25 & 0.19 &  \\
2346.69000 & CO 1 & -0.16 &  &  &  &  \\
2347.59956 & CO 1 & -0.22 &  & 0.23 &  &  \\
2349.07169 & CO 1 & -0.14 &  & 0.25 &  &  \\
2350.58782 & CO 1 & -0.20 &  & 0.04 &  &  \\
2351.84696 & CO 1 & -0.24 &  &  &  & -0.39 \\
2352.04921 & CO 1 &  &  &  &  &  \\
2352.13797 & CO 1 &  &  &  & 0.23 &  \\
2352.29116 & CO 1 & -0.23 &  & 0.25 &  &  \\
2352.40796 & CO 1 &  &  & 0.24 &  &  \\
2352.51600 & CO 1 & -0.37 & -0.00 &  & 0.13 & -0.47 \\
2352.66004 & CO 1 & -0.24 & 0.17 &  &  &  \\
2352.95105 & CO 1 & -0.23 &  &  &  &  \\
2353.08740 & CO 1 & -0.24 & 0.27 & -0.04 &  &  \\
2353.27973 & CO 1 & -0.23 &  & 0.07 &  &  \\
2353.43705 & CO 1 & -0.34 & 0.29 & -0.11 &  &  \\
2353.66739 & CO 1 & -0.20 & 0.21 & -0.02 &  &  \\
2353.74578 & CO 1 & -0.20 & 0.09 & -0.05 & 0.35 &  \\
2353.83083 & CO 1 & -0.25 & 0.37 & 0.38 & 0.38 &  \\
2354.08624 & CO 1 & -0.22 &  &  &  &  \\
2354.26797 & CO 1 & -0.32 &  & 0.07 &  &  \\
2354.55424 & CO 1 & -0.18 &  &  &  &  \\
2354.74345 & CO 1 & -0.15 & 0.30 &  &  &  \\
2355.06660 & CO 1 & -0.17 &  &  &  &  \\
2355.26412 & CO 1 & -0.32 & 0.35 &  &  &  \\
2355.38500 & CO 1 & -0.25 &  &  &  & -0.30 \\
2355.47582 & CO 1 & -0.16 &  &  & 0.24 &  \\
2355.62248 & CO 1 & -0.18 &  & 0.25 &  &  \\
2355.82654 & CO 1 & -0.21 &  &  &  &  \\
2356.22156 & CO 1 & -0.25 &  &  &  &  \\
2356.42898 & CO 1 & -0.21 &  &  &  &  \\
2357.07284 & CO 1 & -0.18 & 0.43 & 0.24 &  & -0.09 \\
2357.55250 & CO 1 & -0.23 &  &  &  &  \\
2357.76413 & CO 1 & -0.26 & 0.31 & -0.00 & 0.45 &  \\
2358.28868 & CO 1 & -0.15 &  & -0.03 &  &  \\
2358.49320 & CO 1 & -0.25 &  &  &  &  \\
2358.79679 & CO 1 & -0.22 & 0.20 & -0.17 &  &  \\
2359.06865 & CO 1 & -0.17 & 0.42 &  &  &  \\
2359.26615 & CO 1 &  &  & -0.04 &  &  \\
2359.89257 & CO 1 & -0.15 &  &  &  &  \\
2360.09086 & CO 1 & -0.19 & 0.27 & -0.16 &  &  \\
2360.56552 & CO 1 & -0.20 &  &  &  &  \\
2360.75932 & CO 1 & -0.03 &  &  &  &  \\
2360.93583 & CO 1 & -0.16 &  &  &  &  \\
2362.37403 & CO 1 & -0.16 &  &  &  &  \\
2362.48043 & CO 1 & -0.14 &  &  &  &  \\
2362.63337 & CO 1 & -0.20 &  &  &  &  \\
2364.22827 & CO 1 & -0.19 &  & -0.16 & 0.20 &  \\
2364.69697 & CO 1 & -0.04 &  &  &  &  \\
2364.78622 & CO 1 &  &  & 0.14 &  &  \\
2364.89693 & CO 1 & -0.15 &  &  &  & -0.30 \\
2365.84856 & CO 1 & -0.17 &  &  &  &  \\
2366.12438 & CO 1 &  &  & 0.09 &  &  \\
2366.95821 & CO 1 & -0.13 &  &  &  &  \\
2367.36259 & CO 1 & -0.17 &  &  &  &  \\
2370.54491 & CO 1 &  &  &  &  & -0.32 \\
2371.82307 & CO 1 & -0.25 &  &  &  &  \\
2372.42223 & CO 1 & -0.09 &  & 0.25 &  & -0.36 \\
2373.14470 & CO 1 &  &  & 0.01 & 0.26 &  \\
2374.50811 & CO 1 & -0.14 &  &  &  &  \\
2375.01914 & CO 1 &  &  &  &  &  \\
2375.91404 & CO 1 & -0.15 &  &  &  &  \\
2377.36344 & CO 1 & -0.21 &  &  &  &  \\
2377.65845 & CO 1 & -0.20 & 0.49 &  &  &  \\
2378.85686 & CO 1 & -0.24 &  &  &  &  \\
2380.37106 & CO 1 & -0.19 &  &  &  &  \\
2380.59797 & CO 1 & -0.16 & 0.29 &  & 0.16 &  \\
2381.96991 & CO 1 & -0.15 &  &  &  &  \\
2382.53184 & CO 1 & -0.33 &  &  &  &  \\
2382.59456 & CO 1 & -0.17 &  &  &  &  \\
2382.69669 & CO 1 & -0.19 &  &  &  & -0.43 \\
2382.79469 & CO 1 & -0.16 &  &  &  &  \\
2382.90301 & CO 1 & -0.29 &  &  &  &  \\
2383.15647 & CO 1 & -0.30 & 0.50 &  &  &  \\
2383.29142 & CO 1 & -0.31 & 0.14 &  &  &  \\
2383.45189 & CO 1 & -0.28 &  & 0.25 & 0.28 &  \\
2383.59790 & CO 1 & -0.22 &  &  &  &  \\
2383.79455 & CO 1 & -0.34 &  &  &  &  \\
2384.17466 & CO 1 & -0.29 &  & 0.03 &  & -0.28 \\
2384.60254 & CO 1 & -0.19 &  &  &  &  \\
2384.83801 & CO 1 & -0.14 &  & 0.17 & 0.14 &  \\
2385.08084 & CO 1 & -0.26 &  &  &  &  \\
2385.25442 & CO 1 & -0.18 &  &  &  &  \\
2385.33719 & CO 1 & -0.11 &  &  &  &  \\
2385.58672 & CO 1 &  &  &  & 0.27 &  \\
2386.47239 & CO 1 & -0.12 &  &  &  &  \\
2386.74069 & CO 1 & -0.13 &  &  &  &  \\
2386.96015 & CO 1 & -0.22 &  & 0.14 &  &  \\
2387.10773 & CO 1 & -0.27 &  &  &  &  \\
2387.38659 & CO 1 &  & 0.40 &  &  &  \\
2387.45112 & CO 1 & -0.18 &  &  &  &  \\
2387.78914 & CO 1 & -0.13 &  &  &  &  \\
2388.07095 & CO 1 & -0.27 &  &  &  &  \\
2388.51950 & CO 1 & -0.10 &  &  &  &  \\
2388.68592 & CO 1 & -0.23 &  &  &  &  \\
2388.79954 & CO 1 & -0.24 & 0.31 & 0.19 &  &  \\
2389.57266 & CO 1 & -0.19 &  & 0.01 &  &  \\
2389.82748 & CO 1 & -0.19 &  & 0.25 & 0.22 &  \\
2390.11294 & CO 1 & -0.14 &  &  &  &  \\
2390.38793 & CO 1 &  &  &  &  & -0.27 \\
2390.50270 & CO 1 & -0.14 & 0.45 &  &  &  \\
2390.97751 & CO 1 & -0.10 &  &  &  &  \\
2391.24627 & CO 1 &  &  & 0.25 &  & -0.42 \\
2391.52835 & CO 1 &  &  & 0.14 &  &  \\
2391.89230 & CO 1 & -0.12 &  &  &  &  \\
2392.24326 & CO 1 &  &  & 0.16 &  & -0.20 \\
2392.84883 & CO 1 & -0.11 &  &  &  &  \\
2394.08266 & CO 1 & -0.14 &  & 0.25 &  &  \\
2394.22269 & CO 1 &  &  &  &  &  \\
2394.44089 & CO 1 & -0.22 &  & 0.13 &  &  \\
2394.70322 & CO 1 & -0.18 &  &  &  & -0.16 \\
2394.90890 & CO 1 & -0.16 &  &  &  &  \\
2395.11769 & CO 1 & -0.18 &  &  &  &  \\
2397.20763 & CO 1 &  &  & 0.17 &  & -0.19 \\
2397.39465 & CO 1 & -0.12 &  &  &  &  \\
2398.46990 & CO 1 & -0.09 &  &  &  &  \\
2399.67285 & CO 1 & -0.05 &  &  &  &  \\
2399.76218 & CO 1 & -0.10 &  &  &  &  \\
1034.38210 & Ca 1 & -0.42 & -0.09 & -0.08 & 0.03 & -0.86 \\
1083.34550 & Ca 1 &  & 0.07 & 0.11 &  &  \\
1083.89886 & Ca 1 &  & -0.02 & 0.01 & -0.06 & -0.39 \\
1086.15956 & Ca 1 & -0.37 &  & 0.03 &  &  \\
1138.14868 & Ca 1 &  &  &  &  & 0.38 \\
1176.75708 & Ca 1 &  &  & -0.09 &  &  \\
1195.59238 & Ca 1 & -0.29 & 0.28 &  & 0.19 & -0.35 \\
1281.60146 & Ca 1 & -0.36 & 0.30 &  &  & -0.47 \\
1282.38059 & Ca 1 & -0.37 &  &  &  & -0.43 \\
1282.70325 & Ca 1 & -0.34 &  & 0.10 &  & -0.45 \\
1288.53198 & Ca 1 &  &  & 0.09 &  &  \\
1290.90699 & Ca 1 & -0.54 & 0.02 & -0.13 & -0.07 & -0.62 \\
1303.35444 & Ca 1 & -0.46 & -0.04 & 0.02 & -0.06 &  \\
1305.78710 & Ca 1 & -0.38 & 0.25 & 0.12 &  &  \\
1308.64157 & Ca 1 &  &  &  &  &  \\
1313.49321 & Ca 1 & -0.47 &  & -0.01 & 0.08 & -0.40 \\
1613.68267 & Ca 1 &  & -0.06 & -0.10 & -0.16 &  \\
1615.07332 & Ca 1 &  & -0.12 & -0.15 &  &  \\
1615.52723 & Ca 1 &  &  & -0.37 &  &  \\
1615.73037 & Ca 1 &  & -0.39 & -0.35 &  &  \\
1619.70136 & Ca 1 & -0.43 & -0.08 & 0.02 & 0.11 &  \\
1620.40741 & Ca 1 &  &  & 0.07 &  &  \\
1981.49671 & Ca 1 & -0.50 &  &  &  &  \\
1985.30034 & Ca 1 &  &  &  &  &  \\
1991.71313 & Ca 1 &  &  &  &  &  \\
1993.36275 & Ca 1 & -0.49 &  &  &  &  \\
1996.17634 & Ca 1 & -0.51 &  & -0.37 &  &  \\
2260.79410 & Ca 1 & -0.32 & 0.47 &  &  &  \\
2262.49412 & Ca 1 & -0.42 & 0.14 &  &  &  \\
2265.12308 & Ca 1 & -0.38 &  &  &  &  \\
973.03268 & Cr 1 & -0.41 &  & 0.05 &  &  \\
973.45792 & Cr 1 &  &  &  &  & -0.00 \\
990.09119 & Cr 1 & -0.23 &  &  &  &  \\
994.90655 & Cr 1 & -0.11 &  &  &  &  \\
1008.03541 & Cr 1 & -0.36 &  &  &  &  \\
1048.62540 & Cr 1 & -0.51 & 0.09 & -0.16 & -0.11 &  \\
1051.00171 & Cr 1 & -0.45 &  & -0.06 & 0.04 & -0.34 \\
1064.76438 & Cr 1 & -0.42 & 0.17 & -0.02 & -0.04 & -0.44 \\
1066.75149 & Cr 1 & -0.43 & 0.19 &  & 0.04 &  \\
1067.21443 & Cr 1 & -0.44 & 0.15 & 0.03 &  & -0.22 \\
1080.13800 & Cr 1 & -0.45 & 0.06 & 0.03 &  &  \\
1081.68853 & Cr 1 &  & 0.15 &  &  &  \\
1082.16614 & Cr 1 & -0.47 & 0.13 & -0.05 & -0.06 &  \\
1090.57128 & Cr 1 & -0.37 & 0.25 & 0.02 & 0.06 &  \\
1101.55268 & Cr 1 & -0.35 &  &  & 0.13 & -0.21 \\
1115.69544 & Cr 1 & -0.30 & 0.36 & 0.03 & 0.20 & -0.43 \\
1131.07280 & Cr 1 & -0.40 & 0.11 & -0.09 & -0.07 &  \\
1133.19405 & Cr 1 &  & 0.21 &  &  &  \\
1133.91605 & Cr 1 & -0.36 &  &  &  &  \\
1137.93347 & Cr 1 & -0.37 &  &  &  &  \\
1139.07563 & Cr 1 &  & 0.24 & 0.04 & 0.11 & -0.19 \\
1139.80608 & Cr 1 & -0.40 &  & -0.04 &  &  \\
1147.30233 & Cr 1 & -0.47 &  &  &  &  \\
1148.46222 & Cr 1 & -0.51 & 0.05 &  & 0.09 & -0.50 \\
1161.05589 & Cr 1 & -0.51 & 0.13 & -0.22 & -0.01 & -0.57 \\
1253.28329 & Cr 1 & -0.39 & 0.12 &  & 0.01 &  \\
1291.00934 & Cr 1 & -0.45 & 0.12 & -0.06 & -0.03 &  \\
1293.70259 & Cr 1 & -0.40 & 0.07 & 0.02 & 0.01 & -0.39 \\
1320.11542 & Cr 1 & -0.43 & 0.14 & -0.10 & -0.05 &  \\
1321.70278 & Cr 1 & -0.39 &  & -0.04 &  &  \\
1434.84617 & Cr 1 & -0.42 &  &  &  &  \\
2023.89085 & Cr 1 & -0.26 &  &  &  &  \\
973.85471 & Fe 1 &  &  & -0.03 &  &  \\
976.38919 & Fe 1 & -0.04 &  &  &  &  \\
980.03298 & Fe 1 & -0.42 &  & 0.02 &  &  \\
983.41588 & Fe 1 & -0.44 &  &  &  &  \\
988.90237 & Fe 1 & -0.18 &  &  &  &  \\
1006.50411 & Fe 1 & -0.39 &  & 0.00 &  &  \\
1008.13959 & Fe 1 & -0.20 &  &  &  &  \\
1008.62386 & Fe 1 & 0.12 &  &  &  &  \\
1011.40567 & Fe 1 & -0.19 &  &  &  &  \\
1014.55585 & Fe 1 & -0.44 & 0.08 & 0.14 &  &  \\
1015.51666 & Fe 1 & -0.41 &  &  &  &  \\
1016.74732 & Fe 1 & -0.42 &  &  &  &  \\
1019.51082 & Fe 1 & -0.24 &  &  &  &  \\
1021.63151 & Fe 1 & -0.44 &  & 0.06 &  &  \\
1021.83913 & Fe 1 & -0.42 &  &  &  &  \\
1026.52097 & Fe 1 & -0.25 &  &  &  &  \\
1034.08878 & Fe 1 & -0.49 & -0.04 & -0.10 & -0.09 &  \\
1034.79607 & Fe 1 & -0.39 &  &  &  &  \\
1037.89996 & Fe 1 & -0.41 & 0.15 & 0.00 &  &  \\
1039.57996 & Fe 1 &  & 0.00 & -0.15 & -0.05 &  \\
1042.30466 & Fe 1 & -0.34 &  & 0.07 &  & -0.22 \\
1042.38116 & Fe 1 & -0.51 & 0.13 &  &  & -0.30 \\
1046.96730 & Fe 1 &  & -0.33 & -0.16 & -0.13 & -0.39 \\
1053.21362 & Fe 1 &  &  & 0.04 &  & -0.04 \\
1057.71371 & Fe 1 & -0.34 &  &  &  &  \\
1061.67330 & Fe 1 & -0.46 & 0.17 &  &  &  \\
1072.51995 & Fe 1 & -0.41 &  &  &  &  \\
1078.30506 & Fe 1 & -0.56 & 0.01 & -0.17 & -0.13 & -0.68 \\
1081.82962 & Fe 1 & -0.48 & 0.11 & -0.08 & -0.16 &  \\
1088.17590 & Fe 1 & -0.26 & 0.34 & 0.11 &  &  \\
1088.42819 & Fe 1 &  & 0.24 &  & -0.04 &  \\
1089.62914 & Fe 1 &  & -0.19 & -0.17 & -0.15 &  \\
1111.97998 & Fe 1 &  & -0.11 & -0.41 & -0.13 &  \\
1114.92599 & Fe 1 & -0.15 &  &  &  &  \\
1125.11204 & Fe 1 &  & -0.09 &  & 0.16 &  \\
1129.88810 & Fe 1 &  &  & -0.20 &  & -0.42 \\
1137.40808 & Fe 1 &  &  & -0.24 & -0.13 &  \\
1142.23193 & Fe 1 &  & 0.05 & -0.14 &  & -0.72 \\
1143.91471 & Fe 1 &  & -0.10 &  &  &  \\
1159.35936 & Fe 1 &  &  &  &  & -0.78 \\
1160.75771 & Fe 1 &  & -0.07 & -0.16 &  & -0.87 \\
1163.82663 & Fe 1 &  & -0.14 & -0.31 &  & -0.53 \\
1178.32768 & Fe 1 &  & -0.19 & -0.35 &  & -0.85 \\
1188.28471 & Fe 1 &  & -0.29 & -0.33 & -0.09 & -0.93 \\
1188.40834 & Fe 1 &  & -0.14 & -0.27 & -0.07 & -0.84 \\
1197.30497 & Fe 1 &  & -0.16 & -0.33 &  & -0.86 \\
1205.30620 & Fe 1 & -0.19 &  &  &  &  \\
1211.94665 & Fe 1 & -0.26 &  &  &  &  \\
1222.71300 & Fe 1 & -0.29 &  &  &  &  \\
1234.04779 & Fe 1 & 0.02 &  &  &  &  \\
1255.70023 & Fe 1 &  & -0.19 & -0.42 &  &  \\
1263.87013 & Fe 1 & -0.41 &  &  &  &  \\
1264.87316 & Fe 1 & -0.32 &  &  &  &  \\
1280.71571 & Fe 1 & -0.38 &  &  &  &  \\
1282.48563 & Fe 1 & 0.09 &  &  &  &  \\
1287.97688 & Fe 1 & -0.56 & -0.11 & -0.22 &  & -0.64 \\
1300.66799 & Fe 1 & 0.05 &  &  &  &  \\
1326.07026 & Fe 1 & -0.45 &  &  &  &  \\
1335.21403 & Fe 1 & -0.16 &  &  &  &  \\
1338.94152 & Fe 1 & -0.26 &  &  &  &  \\
1339.20546 & Fe 1 & -0.25 &  &  &  &  \\
1366.79916 & Fe 1 & -0.38 &  &  &  &  \\
1389.71262 & Fe 1 & -0.22 &  &  &  &  \\
1429.22950 & Fe 1 & -0.52 &  &  &  &  \\
1443.75530 & Fe 1 & -0.41 &  &  &  &  \\
1451.21537 & Fe 1 & -0.45 &  &  &  &  \\
1455.49957 & Fe 1 & -0.53 &  &  &  &  \\
1456.58956 & Fe 1 & -0.49 &  &  &  &  \\
1474.97858 & Fe 1 & -0.37 &  &  &  &  \\
1481.47187 & Fe 1 & -0.31 &  &  &  &  \\
1482.63766 & Fe 1 & -0.58 &  & -0.06 &  &  \\
1495.61398 & Fe 1 & -0.35 &  &  &  &  \\
1498.87293 & Fe 1 & -0.24 &  &  &  &  \\
1519.44734 & Fe 1 & -0.25 &  &  &  &  \\
1520.74653 & Fe 1 & -0.48 & 0.19 & 0.08 & 0.09 &  \\
1529.45216 & Fe 1 & -0.53 & 0.05 & -0.09 & -0.06 &  \\
1559.14745 & Fe 1 & -0.32 &  &  &  &  \\
1562.16218 & Fe 1 & -0.49 & -0.12 & -0.25 &  &  \\
1563.19020 & Fe 1 & -0.38 &  & 0.11 &  &  \\
1564.84361 & Fe 1 & -0.33 &  &  &  &  \\
1566.19483 & Fe 1 & -0.42 &  &  &  &  \\
1569.18838 & Fe 1 & -0.35 &  &  &  &  \\
1569.26353 & Fe 1 & -0.31 &  &  &  &  \\
1581.81171 & Fe 1 & -0.54 & -0.18 & -0.19 &  &  \\
1600.95339 & Fe 1 & -0.37 &  &  &  &  \\
1604.26988 & Fe 1 & -0.36 &  &  &  &  \\
1615.31642 & Fe 1 & -0.26 &  &  &  &  \\
1616.50048 & Fe 1 & -0.38 &  &  &  &  \\
1631.63624 & Fe 1 & -0.38 &  & -0.05 &  &  \\
1632.44002 & Fe 1 & -0.23 &  &  &  &  \\
1644.47610 & Fe 1 &  &  & -0.07 &  &  \\
1651.72373 & Fe 1 & -0.37 &  &  &  &  \\
1664.58308 & Fe 1 & -0.46 &  &  &  &  \\
1784.59517 & Fe 1 & -0.35 &  &  &  &  \\
1963.52215 & Fe 1 & -0.48 &  &  &  &  \\
1992.32837 & Fe 1 & -0.19 &  &  &  &  \\
2034.97227 & Fe 1 & -0.61 &  &  &  &  \\
2225.71007 & Fe 1 & -0.33 &  &  &  &  \\
2238.07229 & Fe 1 & -0.43 &  & 0.04 &  &  \\
2261.98250 & Fe 1 & -0.27 &  & 0.08 &  &  \\
2351.02288 & Fe 1 & 0.17 &  &  &  &  \\
1101.98586 & K 1 &  &  & 0.46 & 0.37 &  \\
1102.26380 & K 1 &  & 0.24 &  &  &  \\
1176.96451 & K 1 & -0.23 & 0.12 & 0.22 & -0.13 & -0.56 \\
1177.28450 & K 1 & -0.31 & 0.00 & 0.07 &  &  \\
1243.22413 & K 1 & -0.21 & 0.04 & 0.12 & 0.18 & -0.59 \\
1252.21014 & K 1 &  & 0.12 & 0.15 &  & -0.56 \\
1516.30504 & K 1 & -0.37 &  & -0.13 &  &  \\
1081.10807 & Mg 1 &  & 0.23 & -0.08 &  &  \\
1095.72500 & Mg 1 & -0.23 &  &  &  &  \\
1096.53956 & Mg 1 &  & 0.42 &  &  &  \\
1182.81637 & Mg 1 & -0.03 & 0.04 & -0.10 & 0.19 & -0.44 \\
1487.75989 & Mg 1 &  &  &  &  &  \\
1502.50010 & Mg 1 &  &  & -0.24 & -0.26 &  \\
1504.02263 & Mg 1 &  &  & 0.00 & -0.12 &  \\
1504.77004 & Mg 1 & -0.30 & 0.36 & -0.19 &  &  \\
1574.06955 & Mg 1 & -0.32 & 0.09 & 0.02 &  &  \\
1574.89497 & Mg 1 & -0.46 & -0.25 & -0.06 & -0.04 &  \\
1576.57936 & Mg 1 & -0.33 &  & 0.06 & -0.05 &  \\
1587.94861 & Mg 1 & -0.23 &  &  &  &  \\
1710.86024 & Mg 1 &  & -0.10 & -0.29 &  &  \\
1289.97678 & Mn 1 & -0.27 & 0.39 & 0.11 & 0.39 & -0.75 \\
1297.59309 & Mn 1 & 0.04 & 0.58 & 0.19 & 0.43 & -0.53 \\
1328.15059 & Mn 1 & -0.07 &  & 0.26 & 0.27 &  \\
1329.38186 & Mn 1 & -0.32 & 0.35 & 0.18 & 0.28 &  \\
1331.89981 & Mn 1 & -0.35 & 0.31 & 0.03 &  &  \\
1362.67522 & Mn 1 &  &  &  &  &  \\
1386.41953 & Mn 1 & -0.13 &  &  &  &  \\
1515.91127 & Mn 1 & -0.32 &  &  &  &  \\
1521.76756 & Mn 1 & -0.37 &  & -0.13 &  &  \\
1526.23763 & Mn 1 & -0.38 &  &  &  &  \\
1074.64399 & Na 1 & -0.29 & 0.24 & 0.22 & 0.14 &  \\
1074.90411 & Na 1 &  &  &  &  & -0.35 \\
1083.48570 & Na 1 & -0.25 &  & 0.27 & 0.27 &  \\
1231.14314 & Na 1 &  & 0.29 &  &  &  \\
1231.99737 & Na 1 &  & 0.21 & 0.22 &  &  \\
1267.91257 & Na 1 & -0.33 &  &  & 0.22 &  \\
2205.64188 & Na 1 & -0.21 &  &  &  &  \\
2208.36759 & Na 1 & -0.18 &  &  &  &  \\
2337.91319 & Na 1 & -0.33 &  &  &  & -0.48 \\
1019.32583 & Ni 1 & -0.24 &  &  &  &  \\
1033.02311 & Ni 1 & -0.14 &  &  &  &  \\
1037.85979 & Ni 1 & -0.21 &  &  &  &  \\
1119.67677 & Ni 1 & -0.27 &  &  &  &  \\
1293.23370 & Ni 1 & -0.60 &  & -0.04 &  &  \\
1696.30721 & Ni 1 &  &  &  &  &  \\
1700.09414 & Ni 1 & -0.40 &  &  &  &  \\
1514.57599 & OH 1 & -0.27 & 0.15 & -0.08 & -0.04 & -0.25 \\
1514.79430 & OH 1 & -0.28 & 0.20 & -0.07 &  &  \\
1527.85139 & OH 1 & -0.28 & 0.16 & -0.07 & 0.16 & -0.25 \\
1528.10492 & OH 1 & -0.27 & 0.13 & -0.14 & 0.00 &  \\
1540.91622 & OH 1 & -0.28 & 0.21 & -0.13 & -0.00 & -0.25 \\
1541.94487 & OH 1 &  & 0.20 &  &  &  \\
1556.02440 & OH 1 & -0.28 & -0.06 & -0.06 &  & -0.96 \\
1556.87731 & OH 1 & -0.28 & 0.22 & -0.06 & 0.12 & -0.25 \\
1557.20818 & OH 1 & -0.28 & 0.07 & -0.11 &  & -0.25 \\
1571.71083 & OH 1 &  &  & -0.39 &  &  \\
1571.96852 & OH 1 & -0.29 & 0.19 & -0.02 & -0.01 & -0.35 \\
1573.04300 & OH 1 & -0.28 & 0.15 & -0.06 & 0.11 & -0.25 \\
1577.87801 & OH 1 & -0.26 & 0.20 & -0.09 &  & -0.25 \\
1588.48902 & OH 1 & -0.26 & 0.15 & -0.21 &  & -0.46 \\
1588.78783 & OH 1 &  & 0.16 & -0.08 &  &  \\
1589.21363 & OH 1 &  & 0.10 & -0.10 &  &  \\
1589.76922 & OH 1 &  & 0.15 & -0.10 &  & -0.25 \\
1603.68674 & OH 1 & -0.28 &  & -0.07 & 0.19 & -0.38 \\
1603.85366 & OH 1 & -0.28 & 0.15 & -0.11 &  & -0.82 \\
1605.27693 & OH 1 & -0.28 & 0.22 & -0.00 & -0.01 & -0.25 \\
1605.54581 & OH 1 &  & 0.13 & -0.17 &  &  \\
1606.16990 & OH 1 &  & 0.12 & -0.16 &  &  \\
1606.50460 & OH 1 & -0.30 & 0.15 & -0.08 &  &  \\
1607.41539 & OH 1 & -0.28 & 0.15 & -0.42 &  &  \\
1619.01472 & OH 1 & -0.27 & 0.14 & -0.05 & 0.02 & -0.50 \\
1619.21192 & OH 1 & -0.30 & 0.19 & -0.10 & 0.06 & -0.37 \\
1620.71680 & OH 1 &  & -0.05 & -0.35 &  &  \\
1625.49575 & OH 1 &  & 0.50 &  &  &  \\
1626.01405 & OH 1 &  &  & -0.04 &  &  \\
1635.22009 & OH 1 & -0.26 & 0.19 &  & 0.12 &  \\
1636.45910 & OH 1 &  & 0.17 & -0.03 &  &  \\
1636.81229 & OH 1 & -0.28 & 0.61 & -0.06 & 0.60 & -0.25 \\
1652.34999 & OH 1 &  & 0.17 & -0.42 &  &  \\
1652.62373 & OH 1 & -0.28 & 0.17 & -0.06 & 0.10 & -0.31 \\
1653.45766 & OH 1 & -0.28 & 0.16 & -0.08 & 0.07 & -0.33 \\
1653.85781 & OH 1 & -0.27 & -0.16 & -0.65 & -0.34 & -0.50 \\
1670.43531 & OH 1 & -0.26 & 0.14 & -0.12 & -0.00 & -0.36 \\
1671.43637 & OH 1 & -0.27 & 0.13 & -0.06 & 0.08 & -0.38 \\
1689.51770 & OH 1 & -0.25 & 0.15 & -0.06 & 0.06 & -0.25 \\
1690.42647 & OH 1 & -0.28 & 0.12 & -0.13 & 0.00 & 0.00 \\
1690.92804 & OH 1 & -0.28 & 0.15 & -0.07 & -0.03 & 0.00 \\
1709.63835 & OH 1 & -0.26 & 0.13 & -0.08 & 0.05 & -0.64 \\
1710.03601 & OH 1 & -0.28 & 0.19 & -0.08 & 0.00 & -0.00 \\
1710.47177 & OH 1 & -0.26 & 0.22 & -0.08 &  &  \\
1711.02097 & OH 1 &  & 0.11 & -0.11 &  &  \\
1730.84380 & OH 1 & -0.29 & -0.20 & -0.08 &  &  \\
1731.29728 & OH 1 & -0.26 & 0.18 & -0.20 & 0.09 &  \\
1731.61100 & OH 1 & -0.25 & -0.49 &  &  &  \\
1732.22403 & OH 1 & -0.27 & 0.18 & -0.01 &  &  \\
1753.89310 & OH 1 &  & 0.21 &  &  &  \\
2205.20065 & Sc 1 & -0.26 &  &  &  &  \\
2206.52923 & Sc 1 & -0.30 &  & -0.17 &  &  \\
2226.66986 & Sc 1 &  &  & 0.01 &  &  \\
1028.89387 & Si 1 & -0.32 &  &  &  &  \\
1037.12562 & Si 1 & -0.31 &  &  &  &  \\
1058.51318 & Si 1 & -0.33 &  &  &  &  \\
1060.34454 & Si 1 & -0.31 & 0.18 &  &  &  \\
1066.09572 & Si 1 & -0.32 &  & -0.14 &  &  \\
1069.42387 & Si 1 & 0.02 &  &  &  &  \\
1072.73928 & Si 1 & -0.01 &  &  &  &  \\
1074.93287 & Si 1 & -0.24 &  & 0.16 &  & -0.42 \\
1078.68582 & Si 1 & -0.27 &  & -0.02 &  &  \\
1084.38346 & Si 1 & -0.00 &  &  &  &  \\
1086.95253 & Si 1 & -0.24 & 0.11 & -0.17 & 0.09 &  \\
1088.53225 & Si 1 & -0.32 &  &  &  &  \\
1097.93032 & Si 1 & -0.35 &  &  &  &  \\
1098.45382 & Si 1 & -0.17 &  &  &  &  \\
1118.75943 & Si 1 & -0.21 &  &  &  &  \\
1198.41985 & Si 1 & -0.36 & 0.27 &  & 0.03 &  \\
1199.15342 & Si 1 & -0.29 &  & -0.14 &  &  \\
1203.15001 & Si 1 & -0.35 & 0.25 & -0.27 & -0.02 &  \\
1210.35746 & Si 1 & -0.34 &  & -0.03 &  &  \\
1227.06788 & Si 1 & -0.32 &  & -0.08 &  &  \\
1239.58153 & Si 1 & -0.22 &  &  &  &  \\
1310.20427 & Si 1 & -0.23 &  &  &  &  \\
1330.90829 & Si 1 & -0.21 &  &  &  &  \\
1332.55755 & Si 1 & -0.43 &  &  &  &  \\
1407.33127 & Si 1 & 0.15 &  &  &  &  \\
1422.44909 & Si 1 & -0.10 &  &  &  &  \\
1588.83177 & Si 1 & -0.33 &  &  &  &  \\
1605.99079 & Si 1 &  &  &  &  &  \\
1621.56717 & Si 1 & -0.15 &  &  &  &  \\
1668.07454 & Si 1 & -0.22 &  &  &  &  \\
1682.81084 & Si 1 & -0.21 &  &  &  &  \\
1732.72967 & Si 1 & -0.35 &  &  &  &  \\
1943.29537 & Si 1 &  &  &  &  &  \\
1972.25063 & Si 1 & -0.27 &  &  &  &  \\
970.56740 & Ti 1 & -0.49 &  & -0.11 & 0.04 & -0.81 \\
971.89677 & Ti 1 & -0.59 & -0.20 & -0.31 & -0.22 & -0.72 \\
972.84198 & Ti 1 & -0.54 &  & -0.30 & -0.12 &  \\
974.36173 & Ti 1 & -0.56 &  & -0.09 &  &  \\
974.69228 & Ti 1 & -0.40 &  &  &  & -0.54 \\
977.03115 & Ti 1 &  & -0.17 & -0.46 & 0.01 & -0.79 \\
978.77015 & Ti 1 &  & -0.06 & 0.04 &  & -0.68 \\
983.21526 & Ti 1 &  & 0.15 & -0.18 & -0.03 & -0.63 \\
987.95924 & Ti 1 & -0.19 &  &  &  &  \\
992.73882 & Ti 1 & -0.30 &  & -0.18 & 0.16 &  \\
994.13930 & Ti 1 & -0.18 &  & 0.10 &  &  \\
999.79489 & Ti 1 & -0.19 &  &  &  &  \\
1000.31050 & Ti 1 & -0.25 & 0.13 & 0.06 &  & -0.48 \\
1001.17517 & Ti 1 & -0.21 & 0.25 & 0.10 &  &  \\
1003.44841 & Ti 1 & -0.43 &  & -0.18 & 0.07 &  \\
1004.88335 & Ti 1 & -0.41 & 0.04 & -0.21 & -0.14 & -0.66 \\
1005.99070 & Ti 1 & -0.42 & -0.09 & -0.17 & -0.12 &  \\
1006.65211 & Ti 1 & -0.18 &  &  & 0.13 & -0.40 \\
1012.09020 & Ti 1 & -0.24 &  & 0.16 &  & -0.20 \\
1039.68123 & Ti 1 & -0.52 & -0.12 & -0.35 & -0.09 & -0.76 \\
1046.00648 & Ti 1 & -0.38 &  & -0.05 & 0.03 &  \\
1049.61245 & Ti 1 & -0.45 & -0.02 & -0.39 & -0.01 & -0.63 \\
1055.29730 & Ti 1 & -0.42 & 0.03 &  &  &  \\
1058.46477 & Ti 1 & -0.48 & -0.08 & -0.45 & -0.02 & -0.77 \\
1060.77323 & Ti 1 & -0.55 & -0.05 & -0.30 &  & -0.84 \\
1066.16351 & Ti 1 & -0.44 & -0.02 & -0.29 & 0.02 & -0.66 \\
1067.70570 & Ti 1 & -0.50 & -0.06 & -0.26 &  &  \\
1072.63954 & Ti 1 & -0.43 & 0.04 & -0.19 & 0.07 & -0.61 \\
1073.28739 & Ti 1 & -0.49 & -0.06 & -0.36 & -0.11 & -0.73 \\
1077.48717 & Ti 1 &  & 0.10 & -0.19 & -0.02 & -0.58 \\
1178.05534 & Ti 1 & -0.40 & 0.03 & -0.19 & 0.01 & -0.45 \\
1179.71824 & Ti 1 & -0.38 & 0.11 & -0.16 & -0.01 &  \\
1194.95446 & Ti 1 &  & 0.11 & -0.27 &  & -0.73 \\
1197.38402 & Ti 1 &  &  & -0.28 &  &  \\
1260.02736 & Ti 1 & -0.36 &  &  & 0.01 & -0.48 \\
1267.10948 & Ti 1 & -0.36 &  &  &  &  \\
1273.83863 & Ti 1 & -0.24 &  &  &  &  \\
1274.49080 & Ti 1 & -0.44 &  &  &  &  \\
1281.14869 & Ti 1 & -0.32 &  &  & -0.01 &  \\
1282.16745 & Ti 1 & -0.31 &  & -0.24 & -0.02 & -0.67 \\
1283.14421 & Ti 1 & -0.38 & 0.05 & -0.19 & -0.04 & -0.63 \\
1284.70386 & Ti 1 & -0.41 & -0.02 & -0.26 & -0.05 & -0.67 \\
1291.99074 & Ti 1 & -0.37 & 0.04 & -0.06 & -0.03 &  \\
1295.08988 & Ti 1 & -0.08 &  &  &  &  \\
1298.75695 & Ti 1 & -0.30 &  &  &  &  \\
1301.18921 & Ti 1 & -0.38 & 0.12 & -0.05 & -0.06 & -0.56 \\
1511.73105 & Ti 1 & -0.34 &  &  &  &  \\
1531.56693 & Ti 1 &  &  &  &  &  \\
1533.48545 & Ti 1 &  & 0.05 & -0.21 & 0.16 &  \\
1554.37594 & Ti 1 & -0.52 & -0.19 & -0.10 & 0.13 &  \\
1560.28410 & Ti 1 & -0.41 & -0.06 & -0.09 & -0.03 &  \\
1569.89818 & Ti 1 &  & 0.00 & -0.14 &  &  \\
1571.55735 & Ti 1 & -0.45 & 0.06 & -0.20 & -0.02 &  \\
1583.68004 & Ti 1 &  & -0.07 & -0.24 &  &  \\
1633.05888 & Ti 1 & -0.18 &  &  &  &  \\
1640.15497 & Ti 1 & -0.34 &  &  &  &  \\
1663.51709 & Ti 1 & -0.45 & 0.01 & -0.14 & -0.10 &  \\
2178.29270 & Ti 1 & -0.29 &  & 0.12 &  &  \\
2189.73820 & Ti 1 & -0.34 & 0.45 &  &  &  \\
2200.44881 & Ti 1 & -0.31 & 0.24 & 0.09 & 0.21 &  \\
2221.12245 & Ti 1 & -0.28 & 0.38 &  &  &  \\
2223.28445 & Ti 1 & -0.31 &  & 0.12 &  & -0.51 \\
2227.40231 & Ti 1 & -0.29 &  &  &  &  \\
2231.06099 & Ti 1 & -0.34 & 0.08 & -0.15 &  &  \\
2244.39008 & Ti 1 & -0.28 &  &  &  &  \\
2296.33316 & Ti 1 & -0.30 & -0.04 &  &  &  \\
2344.14554 & Ti 1 & -0.31 &  &  &  &  \\
1290.11019 & V 1 & -0.16 &  &  &  &  \\
1592.48036 & V 1 &  &  & 0.06 & 0.06 &  \\
\hline
\end{tabular}
\end{table}
